Open Problem: Approximate Planning of POMDPs in the class of Memoryless Policies

Planning plays an important role in the broad class of decision theory. Planning has drawn much attention in recent work in the robotics and sequential decision making areas. Recently, Reinforcement Learning (RL), as an agent-environment interaction problem, has brought further attention to planning methods. Generally in RL, one can assume a generative model, e.g. graphical models, for the environment, and then the task for the RL agent is to learn the model parameters and find the optimal strategy based on these learnt parameters. Based on environment behavior, the agent can assume various types of generative models, e.g. Multi Armed Bandit for a static environment, or Markov Decision Process (MDP) for a dynamic environment. The advantage of these popular models is their simplicity, which results in tractable methods of learning the parameters and finding the optimal policy. The drawback of these models is again their simplicity: these models usually underfit and underestimate the actual environment behavior. For example, in robotics, the agent usually has noisy observations of the environment inner state and MDP is not a suitable model. More complex models like Partially Observable Markov Decision Process (POMDP) can compensate for this drawback. Fitting this model to the environment, where the partial observation is given to the agent, generally gives dramatic performance improvement, sometimes unbounded improvement, compared to MDP. In general, finding the optimal policy for the POMDP model is computationally intractable and fully non convex, even for the class of memoryless policies. The open problem is to come up with a method to find an exact or an approximate optimal stochastic memoryless policy for POMDP models.

==> 3pomdp.tex <==
% !TEX root = master.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LEARNING POMDP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Learning the Parameters of the POMDP}\label{s:learning.pomdp}

%\begin{figure}
%\tiny
%\hspace*{-0.9cm}
%\begin{psfrags}
%\psfrag{x1}[][1]{$x_i$}
%\psfrag{x2}[][1]{$x_{i+1}$}
%\psfrag{x3}[][1]{$x_{i+2}$}
%\psfrag{y1}[][1]{$\vecy_i$}
%\psfrag{y2}[][1]{$\vecy_{i+1}$}
%\psfrag{r1}[][1]{$r_i$}
%\psfrag{r2}[][1]{$r_{i+1}$}
%\psfrag{a1}[][1]{$a_{i}$}
%\psfrag{a2}[][1]{$a_{i+1}$}
%\psfrag{y3}[][1]{$\vecy_{i+2}$}
%\begin{subfigure}{.29\textwidth}
%\hspace*{1cm}
%  \centering
%  \includegraphics[width=.8\linewidth]{figs/HMM.eps}
%  \caption{HMM}
%  \label{fig:HMM}
%\end{subfigure}%
%\begin{subfigure}{.29\textwidth}
%\hspace*{-1cm}
%  \centering
%  \includegraphics[width=.8\linewidth]{figs/MV.eps}
%  \caption{Multi-View}
%  \label{fig:sfig2}
%\end{subfigure}
%\end{psfrags}
%\caption{HMM to Multi-View}
%\label{fig:HMM-MV}
%\end{figure}

In this section we introduce a novel spectral method to estimate the POMDP parameters $f_T$, $f_O$, and $f_R$. A stochastic policy $\pi$ is used to generate a trajectory $(\vec{y}_1, a_1, \vec{r}_1, \ldots, \vec{y}_N, a_N, \vec{r}_N)$ of $\TN$ steps. We need the following assumption that, together with Asm.~\ref{asm:ergodicity}, guarantees that all states and actions are constantly visited.

\begin{assumption}[Policy Set]\label{asm:stochastic.policy}
The policy $\pi$ belongs to $\calP$.
\end{assumption}

Similar to the case of HMMs, the key element to apply the spectral methods is to construct a multi-view model for the hidden states. Despite its similarity, the spectral method developed for HMM by~\cite{anandkumar2014tensor} cannot be directly employed here. In fact, in HMMs the state transition and the observations only depend on the current state. On the other hand, in POMDPs the probability of a transition to state $x'$ not only depends on $x$, but also on action $a$. Since the action is chosen according to a memoryless policy $\pi$ based on the current observation, this creates an indirect dependency of $x'$ on observation $\vec{y}$, which makes the model more intricate.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The multi-view model}\label{ss:multi-view}

We estimate POMDP parameters for each action $l\in [A]$ separately. Let $t\in [2,N-1]$ be a step at which $a_t=l$, we construct three views $(a_{t-1}, \vec{y}_{t-1}, \vec{r}_{t-1})$, $(\vec{y}_t, \vec{r}_t)$, and $(\vec{y}_{t+1})$ which all contain observable elements. As it can be seen in Fig.~\ref{fig:pds2}, all three views provide some information about the hidden state $x_t$ (e.g., the observation $\vec{y}_{t-1}$ triggers the action $a_{t-1}$, which influence the transition to $x_t$). A careful analysis of the graph of dependencies shows that conditionally on $x_t, a_t$ all the views are independent. For instance, let us consider $\vec{y}_{t}$ and $\vec{y}_{t+1}$. These two random variables are clearly dependent since $\vec{y}_t$ influences action $a_t$, which triggers a transition to $x_{t+1}$ that emits an observation $\vec{y}_{t+1}$. Nonetheless, it is sufficient to condition on the action $a_t = l$ to break the dependency and make $\vec{y}_t$ and $\vec{y}_{t+1}$ independent. Similar arguments hold for all the other elements in the views, which can be used to recover the latent variable $x_t$. More formally, we encode the triple $(a_{t-1},\vec{y}_{t-1},\vec{r}_{t-1})$ into a vector $\vec{v}_{1,t}^{(l)}\in \Re^{A\cdot Y\cdot R}$, so that view $\vec{v}_{1,t}^{(l)} = \vec{e}_s$ whenever $a_{t-1}=k$, $\vec{y}_{t-1}=\vec{e}_n$, and $\vec{r}_{t-1}=\vec{e}_m$ for a suitable mapping between the index $s\in\{1,\ldots,A\cdot Y\cdot R\}$ and the indices $(k,n,m)$ of the action, observation, and reward. Similarly, we proceed for $\vec{v}_{2,t}^{(l)}\in\Re^{Y \cdot R}$ and  $\vec{v}_{3,t}^{(l)}\in\Re^{Y}$. We introduce the three view matrices $V^{(l)}_\nu$ with $\nu\in\{1,2,3\}$ associated with action $l$ defined as $V^{(l)}_1\in\Re^{A\cdot Y\cdot R\times X}$, $V^{(l)}_2\in\Re^{Y\cdot R\times X}$, and $V^{(l)}_3\in\Re^{Y\times X}$ such that
%
\begin{align*}%\label{eq:multi.views}
[V_1^{(l)}]_{s,i}&=\Prob\big(\vec{v}_1^{(l)}=\vec{e}_s | x_2=i\big) = [V_1^{(l)}]_{(n,m,k),i} = \Prob\big(\vecy_1=\vec{e}_n,\vec{r}_1=\vec{e}_m,a_1=k|x_2=i\big),\\[0.05in]
[V_2^{(l)}]_{s,i}&=\Prob\big(\vec{v}_2^{(l)}=\vec{e}_s |x_2=i,a_2=l\big) = [V_2^{(l)}]_{(n',m'),i} = \Prob\big(\vecy_2=\vec{e}_{n'},\vec{r}_2=\vec{e}_{m'}|x_2=i,a_2=l\big),\\[0.05in]
[V_3^{(l)}]_{s,i}&=\Prob\big(\vec{v}_3^{(l)}=\vec{e}_s |x_2=i,a_2=l\big) = [V_3^{(l)}]_{n'',i} = \Prob\big(\vecy_3=\vec{e}_{n''}|x_2=i,a_2=l\big).
\end{align*}
%
%%
%\begin{align*}%\label{eq:multi.views}
%[V_1^{(l)}]_{s,i}&=\Prob\big(\vec{v}_1^{(l)}=\vec{e}_s | x_2=i\big) = [V_1^{(l)}]_{(n,m,k),i} \\
%&= \Prob\big(\vecy_1=\vec{e}_n,\vec{r}_1=\vec{e}_m,a_1=k|x_2=i\big),\\
%[V_2^{(l)}]_{s,i}&=\Prob\big(\vec{v}_2^{(l)}=\vec{e}_s |x_2=i,a_2=l\big) = [V_2^{(l)}]_{(n',m'),i}\\
%&= \Prob\big(\vecy_2=\vec{e}_{n'},\vec{r}_2=\vec{e}_{m'}|x_2=i,a_2=l\big),\\
%[V_3^{(l)}]_{s,i}&=\Prob\big(\vec{v}_3^{(l)}=\vec{e}_s |x_2=i,a_2=l\big) = [V_3^{(l)}]_{n'',i}\\
%&= \Prob\big(\vecy_3=\vec{e}_{n''}|x_2=i,a_2=l\big).
%\end{align*}
%%
In the following we denote by $\mu^{(l)}_{\nu,i} = [V_\nu^{(l)}]_{:,i}$ the $i$th column of the matrix $V_\nu^{(l)}$ for any $\nu\in\{1,2,3\}$. Notice that Asm.~\ref{asm:observation} and Asm.~\ref{asm:transition} imply that all the view matrices are full column rank. As a result, we can construct a multi-view model that relates the spectral decomposition of the second and third moments of the (modified) views with the columns of the third view matrix.

%\aacomment{better to put this as a lemma and move derivations to appendix. Many COLT reviewers will know this result. and if they don't they can refer to it in the proof section. Same with recovering parameters of POMDP model. that should be the first lemma saying we can do it and then giving derivations as part of the proof. This is a much better way of explaining.}

\begin{proposition}[Thm. 3.6 in~\citep{anandkumar2014tensor}]\label{lem:spectral.decomposition}
Let $K_{\nu,\nu'}^{(l)} = \E\big[\vec{v}^{(l)}_\nu \otimes \vec{v}^{(l)}_{\nu'}\big]$ be the correlation matrix between views $\nu$ and $\nu'$ and $K^\dagger$ is its pseudo-inverse. We define a modified version of the first and second views as
%
\begin{align}\label{eq:mod.views}
\wt{\vec{v}}_1^{(l)}:=K_{3,2}^{(l)}(K_{1,2}^{(l)})^{\dagger}\vec{v}_1^{(l)}, \quad \wt{\vec{v}}_2^{(l)}:=K_{3,1}^{(l)}(K_{2,1}^{(l)})^{\dagger}\vec{v}_2^{(l)}.
\end{align}
%
Then the second and third moment of the modified views have a spectral decomposition as
%
\begin{align}
M_2^{(l)} &\!\!= \E\big[\wt{\vec{v}}_1^{(l)} \!\otimes \wt{\vec{v}}_2^{(l)}\big] \!=\! \sum_{i=1}^X \omega_\pi^{(l)}(i) \mu^{(l)}_{3,i} \otimes \mu^{(l)}_{3,i},\label{eq:m2}\\
M_3^{(l)} &\!\!= \E\big[\wt{\vec{v}}_1^{(l)} \!\otimes \wt{\vec{v}}_2^{(l)} \!\otimes \vec{v}_3^{(l)}\big] \!=\!\sum_{i=1}^X \omega_\pi^{(l)}(i) \mu^{(l)}_{3,i} \otimes \mu^{(l)}_{3,i} \otimes \mu^{(l)}_{3,i},\label{eq:m3}
\end{align}
%
where $\otimes$ is the tensor product and $\omega_\pi^{(l)}(i) = \Prob[x=i|a=l]$ is the state stationary distribution of $\pi$ conditioned on action $l$ being selected by policy $\pi$.
\end{proposition}

%Although the views are conditionally independent given the middle state and action, we cannot apply the multi-view spectral method yet, because constructing the third moment of the process would lead to a non-symmetric tensor. For this reason, we first need to \textit{symmetrize} the process

Notice that under Asm.~\ref{asm:ergodicity} and~\ref{asm:stochastic.policy}, $\omega_\pi^{(l)}(i)$ is always bounded away from zero.
Given $M_2^{(l)}$ and $M_3^{(l)}$ we can recover the columns of the third view $\mu^{(l)}_{3,i}$ directly applying the standard spectral decomposition method of~\citet{anandkumar2012method}.
% which first uses $M_2^{(l)}$ to whiten the tensor $M_3^{(l)}$ and then proceeds through successive steps of power iteration method and deflation to recover its eigenvalues and eigenvectors. Finally, $\mu^{(l)}_{3,i}$ is recovered by inversion of the whitening matrix.
We need to recover the other views from $V_3^{(l)}$. From the definition of modified views in Eq.~\ref{eq:mod.views} we have
%
\begin{align}\label{eq:expect.mod.views}
\begin{aligned}
\mu^{(l)}_{3,i} = \E\big[\wt{\vec{v}}_1 | x_2 = i,a_2=l \big] = K_{3,2}^{(l)}(K_{1,2}^{(l)})^{\dagger}\E\big[\vec{v}_1| x_2 = i,a_2=l\big] = K_{3,2}^{(l)}(K_{1,2}^{(l)})^{\dagger}\mu^{(l)}_{1,i}, \\ \mu^{(l)}_{3,i} = \E\big[\wt{\vec{v}}_2 | x_2 = i,a_2=l \big] = K_{3,1}^{(l)}(K_{2,1}^{(l)})^{\dagger}\E\big[\vec{v}_2| x_2 = i,a_2=l\big] = K_{3,1}^{(l)}(K_{2,1}^{(l)})^{\dagger}\mu^{(l)}_{2,i}.
\end{aligned}
\end{align}
%
Thus, it is sufficient to invert (pseudo invert) the two equations above to obtain the columns of both the first and second view matrices. This process could be done in any order, e.g., we could first estimate the second view by applying a suitable symmetrization step (Eq.~\ref{eq:mod.views}) and recovering the first and the third views by reversing similar equations to Eq.~\ref{eq:expect.mod.views}. On the other hand, we cannot repeat the symmetrization step multiple times and estimate the views independently (i.e., without inverting Eq.~\ref{eq:expect.mod.views}). In fact, the estimates returned by the spectral method are consistent ``up to a suitable permutation'' on the indexes of the states. While this does not pose any problem in computing one single view, if we estimated two views independently, the permutation may be different, thus making them non-consistent and impossible to use in recovering the POMDP parameters. On the other hand, estimating first one view and recovering the others by inverting Eq.~\ref{eq:expect.mod.views} guarantees the consistency of the labeling of the hidden states.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Recovery of POMDP parameters}\label{ss:recovery}

Once the views $\{V_\nu^{(l)}\}_{\nu=2}^3$ are computed from $M_2^{(l)}$ and $M_3^{(l)}$, we can derive $f_T$, $f_O$, and $f_R$. In particular, all parameters of the POMDP can be obtained by manipulating the second and third view as illustrated in the following lemma.

\begin{lemma}\label{lem:pomdp.parameters}
Given the views $V_2^{(l)}$ and $V_3^{(l)}$, for any state $i\in[X]$ and action $l\in[A]$, the POMDP parameters are obtained as follows. For any reward $m\in[R]$ the reward density is
%
\begin{align}\label{eq:rew.recovery}
f_R(\vec{e}_{m'}|i,l) = \sum_{n'=1}^Y [V_2^{(l)}]_{(n',m'),i};
\end{align}
%
for any observation $n'\in[Y]$ the observation density is
%
\begin{align}
f^{(l)}_O(\vec{e}_{n'}|i) = \sum_{m'=1}^R \frac{[V_2^{(l)}]_{(n',m'),i}}{f_\pi(l|\vec{e}_{n'})\rho(i,l)},\label{eq:obs.recovery}
\end{align}
%
with
%
\begin{align*}%\label{eq:rho.term}
\rho(i,l) = \sum_{m'=1}^R \sum_{n'=1}^Y \frac{[V_2^{(l)}]_{(n',m'),i}}{f_\pi(l|\vec{e}_{n'})} = \frac{1}{\Prob(a_2=l|x_2=i)}.
\end{align*}
%
Finally, each second mode of the transition tensor $T\in\Re^{X\times X\times A}$ is obtained as
%
\begin{align}\label{eq:transition.recovery.inv}
 [T]_{i,:,l} = O^\dagger [V_3^{(l)}]_{:,i},
\end{align}
%
where $O^\dagger$ is the pseudo-inverse of matrix observation $O$ and $f_T(\cdot|i,l) = [T]_{i,:,l}$.
\end{lemma}

In the previous statement we use $f^{(l)}_O$ to denote that the observation model is recovered from the view related to action $l$. While in the exact case, all $f^{(l)}_O$ are identical, moving to the empirical version leads to $A$ different estimates, one for each action view used to compute it. Among them, we will select the estimate with the better accuracy.

\begin{algorithm}[t]
\setstretch{1.1}
\begin{small}
\begin{algorithmic}
\STATE \textbf{Input:}
\STATE $\quad$ Policy density $f_\pi$, number of states $X$
\STATE $\quad$ Trajectory $\langle (\vec{y}_1,a_1,\vec{r}_1), (\vec{y}_2,a_2,\vec{r}_2),\ldots, (\vec{y}_N,a_N, \vec{r}_N)\rangle$

\STATE \textbf{Variables:}
\STATE $\quad$ Estimated second and third views $\wh{V}_2^{(l)}$, and $\wh{V}_3^{(l)}$ for any action $l\in[A]$
\STATE $\quad$ Estimated observation, reward, and transition models $\wh{f}_O$, $\wh{f}_R$, $\wh{f}_T$
\STATE
\FOR{$l=1,\ldots,A$}
\STATE Set $\T(l) = \{t \in [N-1]: a_t = l\}$ and $N(l) = |\T(l)|$
\STATE Construct views $\enspace\vec{v}_{1,t}^{(l)} = (a_{t-1},\vec{y}_{t-1},\vec{r}_{t-1}),$ $\enspace$ $\vec{v}_{2,t}^{(l)} = (\vec{y}_{t},\vec{r}_{t}),$ $\enspace$ $\vec{v}_{3,t}^{(l)} = \vec{y}_{t+1}\quad$ for any $t\in\T(l)$
\STATE Compute covariance matrices $\wh{K}_{3,1}^{(l)}$, $\wh{K}_{2,1}^{(l)}$, $\wh{K}_{3,2}^{(l)}$ as
$$
\wh{K}_{\nu,\nu'}^{(l)} = \frac{1}{N(l)} \sum_{t\in \T(l)} \vec{v}_{\nu,t}^{(l)} \otimes \vec{v}_{\nu',t}^{(l)};  \enspace \nu,\nu'\in\{1,2,3\}
$$
\STATE Compute modified views $\enspace \wt{\vec{v}}_{1,t}^{(l)}:=\wh{K}_{3,2}^{(l)}(\wh{K}_{1,2}^{(l)})^{\dagger}\vec{v}_1, \quad \wt{\vec{v}}_{2,t}^{(l)}:=\wh{K}_{3,1}^{(l)}(\wh{K}_{2,1}^{(l)})^{\dagger}\vec{v}_{2,t}^{(l)}\quad$ for any $t\in\T(l)$

\STATE Compute second and third moments
$$
\wh{M}_2^{(l)} = \frac{1}{N(l)} \sum_{t\in\T_l} \wt{\vec{v}}_{1,t}^{(l)} \otimes \wt{\vec{v}}_{2,t}^{(l)}, \quad
\wh{M}_3^{(l)} = \frac{1}{N(l)} \sum_{t\in\T_l} \wt{\vec{v}}_{1,t}^{(l)} \otimes \wt{\vec{v}}_{2,t}^{(l)} \otimes \vec{v}_{3,t}^{(l)}
$$
\STATE Compute $\wh{V}_3^{(l)}$ = \textsc{\small TensorDecomposition}($\wh{M}_2^{(l)}$, $\wh{M}_3^{(l)}$)
\STATE Compute $\wh{\mu}_{2,i}^{(l)} = \wh{K}_{1,2}^{(l)} (\wh{K}_{3,2}^{(l)})^\dagger \wh{\mu}_{3,i}^{(l)}\quad$ for any $i\in[X]$
\STATE Compute $\wh{f}(\vec{e}_m | i,l) = \sum_{n'=1}^Y [\wh{V}_2^{(l)}]_{(n',m), i}\quad$ for any $i \in [X]$, $m\in [R]$
\STATE Compute $\rho(i,l) = \sum_{m'=1}^R \sum_{n'=1}^Y \frac{[V_2^{(l)}]_{(n',m'),i}}{f_\pi(l | \vec{e}_{n'})}\quad$ for any $i \in [X]$, $n\in[Y]$
\STATE Compute $\wh{f}_O^{(l)}(\vec{e}_{n} | i) = \sum_{m'=1}^R \frac{[V_2^{(l)}]_{(n,m'),i}}{f_\pi(l | \vec{e}_{n}) \rho(i,l)}\quad$ for any $i \in [X]$, $n\in[Y]$
\ENDFOR
\STATE Compute bounds $\B_O^{(l)}$
\STATE Set $l^* = \arg\min_l \B_O^{(l)}$, $\wh{f}_O = \wh{f}_O^{l^*}$ and construct matrix $[\wh{O}]_{n,j} = \wh{f}_O(\vec{e}_n | j)$ 
\STATE Reorder columns of matrices $\wh{V}_2^{(l)}$ and $\wh{V}_3^{(l)}$ such that matrix $O^{(l)}$ and $O^{(l^*)}$ match, $\forall l\in [A]$\footnotemark
\FOR{$i\in[X]$, $l\in[A]$}
\STATE Compute $[T]_{i,:,l} = \wh{O}^\dagger [\wh{V}_3^{(l)}]_{:,i}$
\ENDFOR
\STATE \textbf{Return:} $\wh{f}_R$, $\wh{f}_T$, $\wh{f}_O$, $\B_R$, $\B_T$, $\B_O$
\end{algorithmic}
\end{small}
\caption{Estimation of the POMDP parameters. The routine \textsc{\small TensorDecomposition} refers to the spectral tensor decomposition method of~\citet{anandkumar2012method}.}
\label{alg:spectral.pomdp}
\end{algorithm}
\footnotetext{Each column of $O^{(l)}$ corresponds to $\ell 1$-closest column of $O^{(l^*)}$  }

\paragraph{Empirical estimates of POMDP parameters.}
In practice, $M_2^{(l)}$ and $M_3^{(l)}$ are not available and need to be estimated from samples. Given a trajectory of $N$ steps obtained executing policy $\pi$, let $\T(l) = \{t\in[2,N-1]: a_t = l\}$ be the set of steps when action $l$ is played, then we collect all the triples $(a_{t-1}, \vec{y}_{t-1}, \vec{r}_{t-1})$, $(\vec{y}_t, \vec{r}_t)$ and $(\vec{y}_{t+1})$ for any $t\in\T(l)$ and construct the corresponding views $\vec{v}_{1,t}^{(l)}$, $\vec{v}_{2,t}^{(l)}$, $\vec{v}_{3,t}^{(l)}$. Then we symmetrize the views using empirical estimates of the covariance matrices and build the empirical version of Eqs.~\ref{eq:m2} and~\ref{eq:m3} using $N(l) = |\T(l)|$ samples, thus obtaining
%
\begin{align}
\wh{M}_2^{(l)} = \frac{1}{N(l)} \sum_{t\in\T_l} \wt{\vec{v}}_{1,t}^{(l)} \otimes \wt{\vec{v}}_{2,t}^{(l)}, \quad\quad \wh{M}_3^{(l)} = \frac{1}{N(l)} \sum_{t\in\T_l} \wt{\vec{v}}_{1,t}^{(l)} \otimes \wt{\vec{v}}_{2,t}^{(l)} \otimes \vec{v}_{3,t}^{(l)}.\label{eq:est.m}
\end{align}%\aacomment{Is $N(l)$ not number of triplets where middle action is $l$. }
%
%%
%\begin{align}
%\wh{M}_2^{(l)} &= \frac{1}{N(l)} \sum_{t\in\T_l} \wt{\vec{v}}_{1,t}^{(l)} \otimes \wt{\vec{v}}_{2,t}^{(l)},\label{eq:est.m2}\\
%\wh{M}_3^{(l)} &= \frac{1}{N(l)} \sum_{t\in\T_l} \wt{\vec{v}}_{1,t}^{(l)} \otimes \wt{\vec{v}}_{2,t}^{(l)} \otimes \vec{v}_{3,t}^{(l)}.\label{eq:est.m3}
%\end{align}%\aacomment{Is $N(l)$ not number of triplets where middle action is $l$. }
%%
Given the resulting $\wh{M}_2^{(l)}$ and $\wh{M}_3^{(l)}$, we apply the spectral tensor decomposition method to recover an empirical estimate of the third view $\wh{V}_3^{(l)}$ and invert Eq.~\ref{eq:expect.mod.views} (using estimated covariance matrices) to obtain $\wh{V}_2^{(l)}$. Finally, the estimates $\wh{f}_O$, $\wh{f}_T$, and $\wh{f}_R$ are obtained by plugging the estimated views $\wh{V}_\nu$ in the process described in Lemma~\ref{lem:pomdp.parameters}.\\
Spectral methods indeed recover the factor matrices up to a permutation of the hidden states. In this case, since we separately carry out spectral decompositions for different actions, we recover permuted factor matrices. Since the observation  matrix $O$ is common to all the actions, we use it to align these decompositions.
Let's define $\deltaO$
\begin{align*}
\deltaO=:~\min_{x,x'}\|f_O(\cdot|x)-f_O(\cdot|x')\|_1
\end{align*}

Actually, $\deltaO$ is the minimum separability level of matrix $O$. When the estimation error over columns of matrix O are less than $4\deltaO$, then one can come over the permutation issue by matching columns of $O^{l}$ matrices. In T condition is reflected as a condition that the number of samples for each action has to be larger some number.


 The overall method is summarized in Alg.~\ref{alg:spectral.pomdp}. The empirical estimates of the POMDP parameters enjoy the following guarantee.

\begin{theorem}[Learning Parameters]\label{thm:estimates}
Let $\wh{f}_O$, $\wh{f}_T$, and $\wh{f}_R$ be the estimated POMDP models using a trajectory of $N$ steps. We denote by $\sigma^{(l)}_{\nu,\nu'} = \sigma_X(K_{\nu,\nu'}^{(l)})$ the smallest non-zero singular value of the covariance matrix $K_{\nu,\nu'}$, with $\nu,\nu'\in\{1,2,3\}$, and by $\sigma_{\min}(V_\nu^{(l)})$ the smallest singular value of the view matrix $V_{\nu}^{(l)}$ (strictly positive under Asm.~\ref{asm:observation} and Asm.~\ref{asm:transition}), and we define $\omega_{\min}^{(l)} = \min_{x\in\X} \omega_\pi^{(l)}(x)$ (strictly positive under Asm.~\ref{asm:ergodicity}). If for any action $l\in[A]$, the number of samples $N(l)$ satisfies the condition
%
\begin{align}\label{eq:nl.condition}
N(l) \geq \max\bigg\{\frac{4}{(\sigma_{3,1}^{(l)})^2}, \frac{16C_O^2YR}{{\lambda^{(l)}}^2\deltaO^2}, \left(\frac{G(\pi)\frac{2\sqrt{2}+1}{1-\theta(\pi)}}{{\omega^{(l)}_{\min}\min\limits_{\nu\in\{1,2,3\}}\lbrace\sigma^2_{\min}(V^{(l)}_\nu)\rbrace}}\right)^2\Theta^{(l)}\bigg\} \log\Big(\frac{2(Y^2+AYR)}{\delta}\Big),
\end{align}
%
with $\Theta^{(l)}$, defined in Eq~\ref{eq:nl.condition1}\footnote{We do not report the explicit definition of $\Theta^{(l)}$ here because it contains exactly the same quantities, such as $\omega^{(l)}_{\min}$, that are already present in other parts of the condition of Eq.~\ref{eq:nl.condition}.}, and $G(\pi),\theta(\pi)$ are the geometric ergodicity and the contraction coefficients of the corresponding Markov chain induced by $\pi$, then for any $\delta\in(0,1)$ and for any state $i\in[X]$ and action $l\in[A]$ we have
%
%\begin{small}
%
\begin{align}\label{eq:obs.bound}
\|\wh{f}_O^{(l)}(\cdot|i) \!-\! f_O(\cdot|i)\|_1 \leq \B_O^{(l)} \!:=\frac{ C_O}{\lambda^{(l)}} \sqrt{\frac{YR\log(1/\delta)}{N(l)}},
\end{align}
%
\begin{align}\label{eq:rew.bound}
\|\wh{f}_R(\cdot|i,l) - f_R(\cdot|i,l)\|_1 \leq \B_R^{(l)} := \frac{C_R}{\lambda^{(l)}} \sqrt{\frac{YR\log(1/\delta)}{N(l)}},
\end{align}
%
\begin{align}\label{eq:transition.bound}
\| \wh{f}_T(\cdot|i,l) \!-\! f_T(\cdot|i,l) \|_2 \leq \B_T^{(l)} := \frac{C_T }{\lambda^{(l)}} \sqrt{\frac{YRX^2\log(1/\delta)}{N(l)}},
\end{align}
%
%\end{small}
%
\noindent with probability $1-6(Y^2+AYR)A\delta$ (w.r.t. the randomness in the transitions, observations, and policy), where $C_O$, $C_R$, and $C_T$ are numerical constants and
%
\begin{align}\label{eq:lambda}
\lambda^{(l)} =\sigma_{\min}(O)(\pi_{\min}^{(l)})^2\sigma_{1,3}^{(l)} (\omega^{(l)}_{\min}\min\limits_{\nu\in\{1,2,3\}}\lbrace\sigma^2_{\min}(V^{(l)}_\nu)\rbrace)^{3/2}.
\end{align}
%
Finally, we denote by $\wh{f}_O$ the most accurate estimate of the observation model, i.e., the estimate $\wh{f}_O^{(l^*)}$ such that $l^* = \arg\min_{l\in[A]} \B_O^{(l)}$ and we denote by $\B_O$ its corresponding bound.
\end{theorem}

\noindent\paragraph{Remark 1 (consistency and dimensionality).}
All previous errors decrease with a rate $\wt{O}(1/\sqrt{N(l)})$, showing the consistency of the spectral method, so that if all the actions are repeatedly tried over time, the estimates converge to the true parameters of the POMDP. This is in contrast with EM-based methods which typically get stuck in local maxima and return biased estimators, thus preventing from deriving confidence intervals. 


The bounds in Eqs.~\ref{eq:obs.bound}, \ref{eq:rew.bound}, \ref{eq:transition.bound} on $\wh{f}_O$, $\wh{f}_R$ and  $\wh{f}_T$ depend on $X$, $Y$, and $R$ (and the number of actions only appear in the probability statement). The bound in Eq.~\ref{eq:transition.bound} on  $\wh{f}_T$ is worse than the bounds for $\wh{f}_R$ and $\wh{f}_O$ in Eqs.~\ref{eq:obs.bound}, \ref{eq:rew.bound} by a factor of $X^2$.
 This seems unavoidable since $\wh{f}_R$ and $\wh{f}_O$ are the results of the manipulation of the matrix $V_2^{(l)}$ with $Y\cdot R$ columns, while estimating  $\wh{f}_T$ requires working on both $V_2^{(l)}$ and $V_3^{(l)}$. In addition, to come up with upper bound for $\wh{f}_T$, more complicated bound derivation is needed and it has one step of Frobenious norms to $\ell2$ norm transformation. The derivation procedure for  $\wh{f}_T$ is more complicated compared to $\wh{f}_O$ and $\wh{f}_R$ and adds the term $X$ to the final bound. (Appendix.~\ref{app:proof1})

\noindent\paragraph{Remark 2 (POMDP parameters and policy $\pi$).}
In the previous bounds, several terms depend on the structure of the POMDP and the policy $\pi$ used to collect the samples:
\begin{itemize}
\item $\lambda^{(l)}$ captures the main problem-dependent terms. While $K_{1,2}$ and $K_{1,3}$ are full column-rank matrices (by Asm.~\ref{asm:observation} and~\ref{asm:transition}), their smallest non-zero singular values influence the accuracy of the (pseudo-)inversion in the construction of the modified views in Eq.~\ref{eq:mod.views} and in the computation of the second view from the third using Eq.~\ref{eq:expect.mod.views}. Similarly the presence of $\sigma_{\min}(O)$ is justified by the pseudo-inversion of $O$ used to recover the transition tensor in Eq.~\ref{eq:transition.recovery.inv}. Finally, the dependency on the smallest singular values $\sigma^2_{\min}(V^{(l)}_\nu)$ is due to the tensor decomposition method (see App.~\ref{s:whitening} for more details).
\item A specific feature of the bounds above is that they do not depend on the state $i$ and the number of times it has been explored. Indeed, the inverse dependency on $\omega_{\min}^{(l)}$ in the condition on $N(l)$ in Eq.~\ref{eq:nl.condition} implies that if a state $j$ is poorly visited, then the empirical estimate of any other state $i$ may be negatively affected. This is in striking contrast with the fully observable case where the accuracy in estimating, e.g., the reward model in state $i$ and action $l$, simply depends on the number of times that state-action pair has been explored, even if some other states are never explored at all. This difference is intrinsic in the partial observable nature of the POMDP, where we reconstruct information about the states (i.e., reward, transition, and observation models) only from indirect observations. As a result, in order to have accurate estimates of the POMDP structure, we need to rely on the policy $\pi$ and the ergodicity of the corresponding Markov chain to guarantee that the whole state space is covered.
\item Under Asm.~\ref{asm:ergodicity} the Markov chain $f_{T,\pi}$ is ergodic for any $\pi\in\calP$. Since no assumption is made on the fact that the samples generated from $\pi$ being sampled from the stationary distribution, the condition on $N(l)$ depends on how fast the chain converge to $\omega_\pi$ and this is characterized by the parameters $G(\pi)$ and $\theta(\pi)$.
\item If the policy is deterministic, then some actions would not be explored at all, thus leading to very inaccurate estimations (see e.g., the dependency on $f_\pi(l|\vec{y})$ in Eq.~\ref{eq:obs.recovery}). The inverse dependency on $\pi_{\min}$ (defined in $\calP$) accounts for the amount of exploration assigned to every actions, which determines the accuracy of the estimates. Furthermore, notice that also the singular values $\sigma_{1,3}^{(l)}$ and $\sigma_{1,2}^{(l)}$ depend on the distribution of the views, which in turn is partially determined by the policy $\pi$.
\end{itemize}

Notice that the first two terms are basically the same as in the bounds for spectral methods applied to HMM~\citep{song2013nonparametric}, while the dependency on $\pi_{\min}$ is specific to the POMDP case. On the other hand, in the analysis of HMMs usually there is no dependency on the parameters $G$ and $\theta$ because the samples are assumed to be drawn from the stationary distribution of the chain. Removing this assumption required developing novel results for the tensor decomposition process itself using extensions of matrix concentration inequalities for the case of Markov chain (not yet in the stationary distribution). The overall analysis is reported in App.~\ref{app:ConBound} and~\ref{s:whitening}.



==> App_organization.tex <==
% !TEX root = master.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% PROOF OF SPECTRAL METHOD BOUNDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Organization of the Appendix}\label{app:organization}

\begin{figure}[h!]
\small
\begin{center}
\includegraphics[width=0.8\textwidth]{figs/proofs_new.eps}
\end{center}
\vspace{-0.2in}
\caption{Organization of the proofs.}
\label{fig:proofs}
\end{figure}

We first report the proofs of the main results of the paper in sections~\ref{s:proof.lem:pomdp.parameters}, \ref{app:proof1}, \ref{app:proof2}, \ref{s:proof.remark} and we postpone the technical tools used to derive them from Section~\ref{app:ConBound} on right after preliminary empirical results in Sect.~\ref{s:experiments}. In particular, the main lemmas and theorems of the paper are organized as in Fig.~\ref{fig:proofs}.

Furthermore, we summarize the additional notation used throughout the appendices in the following table.

%\begin{table}[h]\caption{Notation used in the appendix.}
\begin{center}
\begin{tabular}{r c p{12cm} }
\toprule
$\Delta_{n^{(l)}}$ &  & Concentration matrix\\  
$\eta_{i,j}^{(l)}(\cdot,\cdot,\cdot)$ &  & mixing coefficient\\  
$p(i,l)$ &  & translator of $i'th$ element in sequence of samples given middle action $l$ to the actual sequence number \\  
$\HH^{i|l}$ &  & $i'th$ quadruple consequence of states random variable given second action $l$\\  
$\hhh^{i|l}$ &  & $i'th$ quadruple consequence of states given second action $l$\\  
$\HH^{j|l}_i$ &  & sequence of all $\HH^{i'|l}$ for $i'\in\{i,\ldots,j\}$ \\  
$\hhh^{i|l}$ &  & sequence of all $\hhh^{i'|l}$ for $i'\in\{i,\ldots,j\}$\\  
$\VV^{i|l}$ &  & $i'th$ triple consequence of views random variable given second action $l$\\  
$\vv^{i|l}$ &  & $i'th$ triple consequence of observation given second action $l$\\  
$\VV^{j|l}_i$ &  & sequence of all $\VV^{i'|l}$ for $i'\in\{i,\ldots,j\}$ \\  
$\vv^{i|l}$ &  & sequence of all $\vv^{i'|l}$ for $i'\in\{i,\ldots,j\}$\\  
\bottomrule
\end{tabular}
\end{center}
%\label{tab:TableOfNotationForMyResearch3}
%\end{table}
For the tensor $A\in\mathbb{R}^{d_1\times d_2\ldots\times d_p}$, and matrices $\lbrace V_i\in\mathbb{R}^{d_i,n_i}:i\in\lbrace 1,\ldots,p\rbrace\rbrace$, the tensor multi-linear operator is defined as follows\\
For the ${i_1,i_2,\ldots,i_p}-th$ element
\begin{align*}
\left[A(V_1,V_2, \ldots, V_p)\right]_{i_1,i_2,\ldots,i_p}\displaystyle\sum_{j_1,j_2,\ldots,j_p\in\lbrace 1,2,\ldots,p\rbrace}A_{j_1,j_2,\ldots,j_p\in\lbrace 1,2,\ldots,p\rbrace}[V_1]_{j_1,i_1}[V_2]_{j_2,i_2}\cdots[V_p]_{j_p,i_p}
\end{align*}


==> Cextension.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LIMITED MEMORY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Extension to Bounded-Memory Policies}\label{app:bounded.memory}

\begin{figure}[h]
\tiny
\begin{center}
\begin{psfrags}
\psfrag{x1}[][1]{$x_0$}
\psfrag{x2}[][1]{$x_{1}$}
\psfrag{x3}[][1]{$x_{2}$}
\psfrag{x0}[][1]{$x_{-1}$}
\psfrag{y1}[][1]{$\vecy_0$}
\psfrag{y2}[][1]{$\vecy_{1}$}
\psfrag{y0}[][1]{$\vecy_{-1}$}
\psfrag{r1}[][1]{$r_0$}
\psfrag{r2}[][1]{$r_{1}$}
\psfrag{r0}[][1]{$r_{-1}$}
\psfrag{a1}[][1]{$a_{0}$}
\psfrag{a2}[][1]{$a_{1}$}
\psfrag{a0}[][1]{$a_{-1}$}
\includegraphics[width=0.45\textwidth,natwidth=810,natheight=642,trim={0 1.5cm 2cm 0.5cm},clip]{figs/I-6.eps}
\end{psfrags}
\end{center}
\caption{Bounded-Memory POMDP when \past=2.}
\label{fig:I-6}
\end{figure}


Throughout the paper we consider memory-less policies which only consider the current observation to decide which action to take. Nonetheless, our method, and notably the process of estimation of the POMDP parameters, can be easily extended to the case of bounded-memory policies. Let $\pi$ be a policy such that at time $t$ all the past $\past$ observations are considered to decide the action, that is $f_\pi(a|\vec{y}_t, \vec{y}_{t-1},\ldots,\vec{y}_{t-\past})$. In Fig.~\ref{fig:I-6} we illustrate the case for $\past=2$. In this case, we have to redefine the notion of views that we introduced in Sect.~\ref{s:learning.pomdp}. We define the first view $(\vecy_{-(\past-1)},a_{-(\past-1)},r_{-(\past-1)},\ldots,\vecy_{(-1)},a_{(-1)},r_{(-1)})$, the second view $(\vecy_0,r_0)$, and the third view $(\vecy_{(1)},r_{(1)},\ldots,\vecy_{(\past-1)},r_{(\past-1)})$. Given state $x_0$ and all actions $a_0,\ldots,a_{\past-1}$, it is easy to see that these views are independent and the multi-view model can be applied by extending the definitions of $V_{\nu}^{(l)}$ to this case. If the views satisfy the assumption of being full column rank, then all the results presented in Sect.~\ref{s:learning.pomdp} can be easily extended.




Usually, in the real systems, the agents do not make decision at each time step, even they do not apply their decision at each time step because usually making decision and applying that is expensive for agents. Lets take a look at the system that the agent chooses an action based on $p$ previous observation (including current observation) and then for $p-1$ time step, it just looks at the system and records the data, after that, based on this collected data, it choose new action. This model is simpler that the above mentioned model which we are not able to investigate it in this draft.  The simpler model is as follow. Let us consider the case of $p=2$, then
\begin{equation}
\begin{split}
&[\obs_1^{a_0=i}]_{l,f}=Pr(\vecy_{-1}=\vec{e}_j,r_{-1}=\vec{e}_b,a_{-1}=c|x_0=f)\\
&[\obs_2^{a_0=i}]_{l,f}=Pr(\vecy_0=\vec{e}_{j'},r_0=\vec{e}_{b'}|x_0=f,a_0=i)\\
&[\obs_3^{a_2=i}]_{l,f}=Pr(\vecy_1=\vec{e}_j,r_1=\vec{e}_b|x_0=f,a_0=i)
\end{split}
\end{equation}
The full rank condition is satisfied if either $\obs$ matrix or $R$ matrix is full column rank and transition matrix is full rank. Same idea as before, the agent do the learning part for each action and for each of them once it looks at third view as a third effect and once second view as a third view. By this it can learn $\obs$ and $\trans^{(a_0=i)}$ for all $i$. Addition to that, the agent need to find out the transition matrix when during passive time which is for example transition form $x_{-1}$ to $x_0$. To learn this part of model, the agent needs to estimate another set of $\obs$ matrices whose columns are conditioned on $x_1$, $i.e.$:
\begin{equation}
\begin{split}
&[\obs_1]_{l,f}=Pr(\vecy_{0}=\vec{e}_j,r_{0}=\vec{e}_b,a_{0}=c|x_1=f)\\
&[\obs_2]_{l,f}=Pr(\vecy_1=\vec{e}_{j'},r_1=\vec{e}_{b'}|x_1=f)\\
&[\obs_3]_{l,f}=Pr(\vecy_2=\vec{e}_j,r_2=\vec{e}_b,a_2=c|x_1=f)
\end{split}
\end{equation}
this set of $\obs$ gives us the transition matrix.




==> MainTheorem.tex <==
\section{Concentration Bound}\label{app:HMMConst}
\noindent\paragraph{Concentration of functions of a HMM}  We now provide concentration bounds for any matrix valued function $\phi(\cdot)$ over samples drawn from a HMM. This extends the result on scalar functions by~\citet{kontorovich2014uniform}.

For any ergodic Markov chain, lets consider $\omega$ as its stationary distribution and $f_{1\rightarrow t}(x_t|x_1)$ as a distribution over states at time $t$ given initial state $x_1$. Lets define inverse mixing time $\rho_{mix}(t)$ as follows
\begin{align*}
\rho_{mix}(t)=\sup_{x_1}\left\|f_{1\rightarrow t}(\cdot|x_1)-\omega\right\|_{TV}
\end{align*}
~\citet{kontorovich2014uniform} show  that this measure can be bounded by%\aacomment{replace with Roi's paper as ref}
\begin{align*}
\rho_{mix}(t)\leq G\theta^{t-1},
\end{align*}
where $1\leq G<\infty$ is $geometric$ $ergodicity$ and $0\leq \theta<1$ is contraction coefficient of Markov chain.

As before, let  $\bfy^n:=[\vec{y}_1, \ldots, \vec{y}_n]\in \calY^n$ denote the sequence of observations from HMM and let $x^n :=[x_1, \ldots, x_n]\in \calX^n$ denote the sequence of hidden states. We now consider matrix valued function $\Phi:\calY^{n}\rightarrow \mathbb{R}^{d_1\times d_2}$. It is said to be   $c$-Lipschitz  with respect to  spectral norm when
\begin{align*}
\sup_{\bfy^n, {\bfy'}^n \in \calY^n}\frac{\left\|\Phi(\bfy^n)-\Phi({\bfy'}^n)\right\|_2}{\|\bfy^n-{\bfy'}^n\|_H}\leq c
\end{align*}
where $\|\cdot\|_H$ is norm with respect to Hamming metric,   and $\bfy^n, {\bfy'}^n$ are any two sequences of  sample observations.
\begin{theorem}[HMM Concentration Bound]
Consider Hidden Markov Model with finite sequence of $n$ samples $\vec{y}_i$ as observations from finite observation set $\bfy^n$ and arbitrary initial state distribution. For any $c$-Lipschitz matrix valued function $\Phi(\cdot)$, we have
\begin{align*}
\left\|\Phi(\bfy^n)-\mathbb{E}[\Phi(\bfy^n)]\right\|_2\leq G\frac{1+\frac{1}{\sqrt{2}cn^{\frac{3}{2}}}}{1-\theta}\sqrt{8c^2n\log(\frac{(d_1+d_2)}{\delta})}
\end{align*}
with probability at least $1-\delta$, where G is  $geometric$ $ergodicity$ constant of corresponding Markov chain, and the $\mathbb{E}[\Phi(\bfy^n)]$ is expectation over samples of HMM when the initial distribution corresponds to the stationary distribution.
\label{thm:GeneralConcentrationBound}
\end{theorem}
\begin{proof}
In the Appendix. \ref{app:Proof_main}
\end{proof}
%Later, we extend this result  to the more complicated model of memory-less policy POMDP in order to derive our regret bounds. 
\begin{theorem}[POMDP Concentration Bound]
Consider Partially Observable Markov Decision Process with finite sequence of $n(l)$ samples $\vec{y}_i^{(l)}$ for all $i\in\lbrace1,2,\ldots,n(l)\rbrace~\forall l\in[A]$ as observations from finite observation sets $\bfy^{n(l)}$ and arbitrary initial state distribution. For any $c$-Lipschitz matrix valued function $\Phi^l(\cdot)$ function, we have
\begin{align*}
\left\|\Phi^l(\bfy^{n(l)})-\mathbb{E}[\Phi^l(\bfy^{n(l)})]\right\|_2\leq G\frac{1+\frac{1}{\sqrt{2}cn^{\frac{3}{2}}}}{1-\theta}\sqrt{8c^2n\log(\frac{(d_1+d_2)}{\delta})}
\end{align*}
with probability at least $1-\delta$, where G is  $geometric$ $ergodicity$ constant of corresponding Markov chain, and the $\mathbb{E}[\Phi(\bfy^{n(l)})]$ is expectation over samples of POMDP with middle action $l$ when the initial distribution corresponds to the stationary distribution.
\label{thm:GeneralConcentrationBoundPOMDP}
\end{theorem}
\begin{proof}
In the Appendix. \ref{app:Proof_main}
\end{proof}


==> macros.tex <==

%\mbox - function definitions
\def\tl{\tilde}\renewcommand\t{{\scriptscriptstyle\top}}

\newcommand\Dir{\operatorname{Dir}}
\newcommand\inner[1]{\ensuremath{\langle #1 \rangle}}
%\newcommand{\aacomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AA:} \textsf{#1} \#\#\#}}}
\newcommand{\mjcomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# MJ:} \textsf{#1} \#\#\#}}}
\newcommand{\hscomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# HS:} \textsf{#1} \#\#\#}}}
\def\indicator{{1{\hskip -2.5 pt}\hbox{I}}}
\DeclareMathOperator{\polylog}{polylog}
\newcommand\cov{\operatorname{Cov}}
 %\DeclareMathOperator{\short}{short}
\DeclareMathOperator{\sym}{Sym}
  \DeclareMathOperator{\tw}{tw}
  \DeclareMathOperator{\local}{local}
  \DeclareMathOperator{\range}{range}
   \DeclareMathOperator{\Path}{Path}
 \DeclareMathOperator{\Sg}{Sg}
 \DeclareMathOperator{\spt}{SP}
 \DeclareMathOperator{\avg}{avg}
  \DeclareMathOperator{\nbd}{\mathcal{N}}
 \DeclareMathOperator{\parent}{Pa}
 \DeclareMathOperator{\Cq}{Cq}
 \DeclareMathOperator{\TW}{TW}
 

 \DeclareMathOperator{\approxML}{ApproxML}
 \DeclareMathOperator{\Bethe}{Bethe}
 \DeclareMathOperator{\TRW}{TRW}
 \DeclareMathOperator{\conv}{Conv}
 \DeclareMathOperator{\lbp}{LBP}
 \DeclareMathOperator{\Corr}{Corr}
 \DeclareMathOperator{\hCorr}{\widehat{Corr}}
 \DeclareMathOperator{\hSc}{\widehat{\mathcal{S}}}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\mst}{MST}
\DeclareMathOperator{\supp}{supp}
 \DeclareMathOperator{\dtv}{d_{TV}}
 \DeclareMathOperator{\hdtv}{\hd_{TV}}
 \DeclareMathOperator*{\argmin}{arg\,min}
 \DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\rank}{Rank}
\DeclareMathOperator{\Krank}{Rank_K}
\DeclareMathOperator{\Det}{Det}
\DeclareMathOperator{\poiss}{Poiss}
\DeclareMathOperator{\unif}{Unif} \DeclareMathOperator{\Deg}{Deg}
\def\simiid{{\overset{i.i.d.}{\sim}}}
\def\lcv{{\,\,\underset{cv}{\leq}\,\,}}
\def\gcv{{\,\,\underset{cv}{\geq}\,\,}}
\def\lcx{{\,\,\underset{cx}{\leq}\,\,}}
\def\gcx{{\,\,\underset{cx}{\geq}\,\,}}
\def\leqst{{\,\,\overset{st}{\leq}\,\,}}
\def\geqst{{\,\,\overset{st}{\geq}\,\,}}
\def\eqdist{{\,\,\overset{d}{=}\,\,}}
\def\geqrh{{\,\,\overset{rh}{\geq}\,\,}}
\def\geqlr{{\,\,\overset{lr}{\geq}\,\,}}
\def\eqlr{{\,\,\overset{lr}{=}\,\,}}
\def\comment{{\mbox{\bf Comment\_Anima: }}}
\def\tha{{\mbox{\tiny th}}}

\DeclareMathOperator{\Aug}{Aug}
\DeclareMathOperator{\watts}{Watts}
\DeclareMathOperator{\girth}{Girth}
\DeclareMathOperator{\PL}{PL}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\ER}{ER}
\DeclareMathOperator{\reg}{Reg}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\hSigma}{\widehat{\Sigma}}
%\DeclareMathOperator{\hrho}{\widehat{\rho}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Poiss}{Poiss}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\Diam}{Diam}
\def\erf{\mbox{erf}}
\def\erfc{\mbox{erfc}}
\def\qfunc{\mbox{Q}}
%\def\myexp{\mbox{e}}
\def\snr{\mbox{{SNR}}}
\def\signum{\mbox{sgn}}
\def\Card{\mbox{Card}}
\DeclareMathOperator*{\plim}{plim}
\def\convd{\overset{d}\rightarrow}
\def\convp{\overset{p}\rightarrow}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\def\pl{{\parallel}}
%\DeclarePairedDelimiter\norm{\lVert}{\rVert}
%\DeclarePairedDelimiter\nuclearnorm{\lVert}{\rVert_*}
%\DeclarePairedDelimiter\onenorm{\lVert}{\rVert_1}
%\def\rinfnorm{\rVert_{\infty}}
%\DeclarePairedDelimiter\infnorm{\lVert}{\rinfnorm}
%\def\lnorm{{\lvert\!\lvert\!\lvert}}
%\def\rnorm{{\rvert\!\rvert\!\rvert}}
%\DeclarePairedDelimiter\gennorm{\lnorm}{\rnorm}
% \DeclarePairedDelimiter\abs{\lvert}{\rvert}
% \DeclarePairedDelimiter\geninfnorm{\lnorm}{\rnorm_{\infty}}
% \DeclarePairedDelimiter\genonenorm{\lnorm}{\rnorm_{1}}
\DeclareMathOperator{\atanh}{atanh}
 \DeclareMathOperator{\sech}{sech}
 \def\0{{\bf 0}}

\DeclareMathOperator{\lea}{\overset{(a)}{\leq}}
\DeclareMathOperator{\leb}{\overset{(b)}{\leq}}
\DeclareMathOperator{\lec}{\overset{(c)}{\leq}}
\DeclareMathOperator{\led}{\overset{(d)}{\leq}}
\DeclareMathOperator{\lee}{\overset{(e)}{\leq}}

\DeclareMathOperator{\eqa}{\overset{(a)}{=}}
\DeclareMathOperator{\eqb}{\overset{(b)}{=}}
\DeclareMathOperator{\eqc}{\overset{(c)}{=}}
\DeclareMathOperator{\eqd}{\overset{(d)}{=}}
\DeclareMathOperator{\eqe}{\overset{(e)}{=}}

\DeclareMathOperator{\gea}{\overset{(a)}{\geq}}
\DeclareMathOperator{\geb}{\overset{(b)}{\geq}}
\DeclareMathOperator{\gec}{\overset{(c)}{\geq}}
\DeclareMathOperator{\ged}{\overset{(d)}{\geq}}
\DeclareMathOperator{\gee}{\overset{(e)}{\geq}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% \algrenewcommand{\algorithmiccomment}[1]{// #1}
% \algrenewcommand{\algorithmicrequire}{\textbf{Input:}}
% \algrenewcommand{\algorithmicforall}{\textbf{for each}}


%text abbreviations
%\def\etal{{et al. \/}}
\def\viz{{viz.,\ \/}}
\def\ie{{i.e.,\ \/}}
\def\eg{{e.g.,\ \/}}
\def\etc{{etc.  }}
\def\ifff{{iff  }}
\def\as{{a.s.  }}
\def\st{{s.t.  }}
\def\wpone{{w.p.}\,1\,\,}
\def\wpp{{w.p.p.}\,\,}
\def\for{\,\,\mbox{for}\quad}
\def\ifmbox{\,\,\mbox{if}\quad}
\def\nn{\nonumber}
%\def\qed{\hfill$\Box$}
\def\ni{\noindent}

\def\qed{\hfill\hbox{${\vcenter{\vbox{
    \hrule height 0.4pt\hbox{\vrule width 0.4pt height 6pt
    \kern5pt\vrule width 0.4pt}\hrule height 0.4pt}}}$}}
\def\complx{\mathbb{C}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ldp : use ldp.tex file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Detection on Graphs



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%colors
\def\tcr{\textcolor{red}}
\def\tcb{\textcolor{blue}}
\def\tcg{\textcolor{green}}
\def\tcw{\textcolor{white}}
\def\tcm{\textcolor{magenta}}
\def\tccyan{\textcolor{cyan}}
\def\tcv{\textcolor{violet}}
\definecolor{myred}{rgb}{0.3,0.0,0.7}
\definecolor{dkg}{rgb}{0.1,0.7,0.2}
\definecolor{dkb}{rgb}{0.0,0.2,0.8}

\def\tcdkb{\textcolor{dkb}}
\def\tcdkg{\textcolor{dkg}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\mathscr

\newcommand{\Amsc}{\mathscr{A}}
\newcommand{\Cmsc}{\mathscr{C}}
\newcommand{\Dmsc}{\mathscr{D}}
\newcommand{\Emsc}{\mathscr{E}}
\newcommand{\Fmsc}{\mathscr{F}}
\newcommand{\Gmsc}{\mathscr{G}}
\newcommand{\Hmsc}{\mathscr{H}}
\newcommand{\Kmsc}{\mathscr{K}}
\newcommand{\Nmsc}{\mathscr{N}}
\newcommand{\Pmsc}{\mathscr{P}}
\newcommand{\Qmsc}{\mathscr{Q}}
\newcommand{\Rmsc}{\mathscr{R}}
\newcommand{\Smsc}{\mathscr{S}}
\newcommand{\Tmsc}{\mathscr{T}}
\newcommand{\Umsc}{\mathscr{U}}
\newcommand{\Xmsc}{\mathscr{X}}
\newcommand{\Ymsc}{\mathscr{Y}}



%%%%%%%%%%%%%%%%%%%%%%hat
 \def\ha{\hat{a}}
 \def\hb{\hat{b}}
 \def\hc{\hat{c}}
\def\hd{\widehat{d}}
 \def\he{\widehat{e}}
 \def\hf{\hat{f}}
 \def\hg{\widehat{g}}
 \def\hh{\widehat{h}}
 \def\hi{\widehat{i}}
 \def\hj{\widehat{j}}
 \def\hk{\widehat{k}}
 \def\hl{\widehat{l}}
 \def\hm{\widehat{m}}
 \def\hn{\widehat{n}}
 \def\ho{\widehat{o}}
 \def\hp{\widehat{p}}
 \def\hq{\widehat{q}}
 \def\hr{\widehat{r}}
 \def\hs{\widehat{s}}
 \def\hatt{\widehat{t}}
 \def\hu{\hat{u}}
 \def\hv{\widehat{v}}
 \def\hw{\hat{w}}
 \def\hx{\hat{x}}
 \def\hy{\hat{y}}
 \def\hz{\widehat{z}}
% %bold caps
 \def\hA{\hat{A}}
 \def\hB{\hat{B}}
 \def\hC{\hat{C}}
 \def\hD{\widehat{D}}
 \def\hE{\widehat{E}}
 \def\hF{\widehat{F}}
 \def\hG{\widehat{G}}
 \def\hH{\widehat{H}}
 \def\hI{\widehat{I}}
 \def\hJ{\widehat{J}}
 \def\hK{\widehat{K}}
 \def\hL{\widehat{L}}
 \def\hM{\widehat{M}}
\def\hN{\widehat{N}}
 \def\hO{\widehat{O}}
 \def\hP{\widehat{P}}
 \def\hQ{\widehat{Q}}
 \def\hR{\widehat{R}}
 \def\hS{\widehat{S}}
\def\hT{\widehat{T}}
 \def\hU{\widehat{U}}
 \def\hV{\widehat{V}}
\def\hW{\widehat{W}}
 \def\hX{\hat{X}}
 \def\hY{\widehat{Y}}
 \def\hZ{\widehat{Z}}

 \def\hlambda{\widehat{\lambda}}
\def\hpi{\widehat{\pi}}
\def\hnu{\widehat{\nu}}
\def\hbd{\widehat{\mathbf{d}}}


\def\bLambda{\mathbf{\Lambda}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold alphabets
\def\bfzero{{\mathbf{0}}}
\def\bfone{{\mathbf{1}}}
\def\bfa{{\mathbf a}}
\def\bfb{{\mathbf b}}
\def\bfc{{\mathbf c}}
\def\bfd{{\mathbf d}}
\def\bfe{{\mathbf e}}
\def\bff{{\mathbf f}}
\def\bfg{{\mathbf g}}
\def\bfh{{\mathbf h}}
\def\bfi{{\mathbf i}}
\def\bfj{{\mathbf j}}
\def\bfk{{\mathbf k}}
\def\bfl{{\mathbf l}}
\def\bfm{{\mathbf m}}
\def\bfn{{\mathbf n}}
\def\bfo{{\mathbf o}}
\def\bfp{{\mathbf p}}
\def\bfq{{\mathbf q}}
\def\bfr{{\mathbf r}}
\def\bfs{{\mathbf s}}
\def\bft{{\mathbf t}}
\def\bfu{{\mathbf u}}
\def\bfv{{\mathbf v}}
\def\bfw{{\mathbf w}}
\def\bfx{{\mathbf x}}
\def\bfy{{\mathbf y}}
\def\bfz{{\mathbf z}}
%bold caps
\def\bfA{{\mathbf A}}
\def\bfB{{\mathbf B}}
\def\bfC{{\mathbf C}}
\def\bfD{{\mathbf D}}
\def\bfE{{\mathbf E}}
\def\bfF{{\mathbf F}}
\def\bfG{{\mathbf G}}
\def\bfH{{\mathbf H}}
\def\bfI{{\mathbf I}}
\def\bfJ{{\mathbf J}}
\def\bfK{{\mathbf K}}
\def\bfL{{\mathbf L}}
\def\bfM{{\mathbf M}}
\def\bfN{{\mathbf N}}
\def\bfO{{\mathbf O}}
\def\bfP{{\mathbf P}}
\def\bfQ{{\mathbf Q}}
\def\bfR{{\mathbf R}}
\def\bfS{{\mathbf S}}
\def\bfT{{\mathbf T}}
\def\bfU{{\mathbf U}}
\def\bfV{{\mathbf V}}
\def\bfW{{\mathbf W}}
\def\bfX{{\mathbf X}}
\def\bfY{{\mathbf Y}}
\def\bfZ{{\mathbf Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold symbols

\def\alphabf{\hbox{\boldmath$\alpha$\unboldmath}}
\def\betabf{\hbox{\boldmath$\beta$\unboldmath}}
\def\gammabf{\hbox{\boldmath$\gamma$\unboldmath}}
\def\deltabf{\hbox{\boldmath$\delta$\unboldmath}}
\def\epsilonbf{\hbox{\boldmath$\epsilon$\unboldmath}}
\def\zetabf{\hbox{\boldmath$\zeta$\unboldmath}}
\def\etabf{\hbox{\boldmath$\eta$\unboldmath}}
\def\iotabf{\hbox{\boldmath$\iota$\unboldmath}}
\def\kappabf{\hbox{\boldmath$\kappa$\unboldmath}}
\def\lambdabf{\hbox{\boldmath$\lambda$\unboldmath}}
\def\mubf{\hbox{\boldmath$\mu$\unboldmath}}
\def\nubf{\hbox{\boldmath$\nu$\unboldmath}}
\def\xibf{\hbox{\boldmath$\xi$\unboldmath}}
\def\pibf{\hbox{\boldmath$\pi$\unboldmath}}
\def\rhobf{\hbox{\boldmath$\rho$\unboldmath}}
\def\sigmabf{\hbox{\boldmath$\sigma$\unboldmath}}
\def\taubf{\hbox{\boldmath$\tau$\unboldmath}}
\def\upsilonbf{\hbox{\boldmath$\upsilon$\unboldmath}}
\def\phibf{\hbox{\boldmath$\phi$\unboldmath}}
\def\chibf{\hbox{\boldmath$\chi$\unboldmath}}
\def\psibf{\hbox{\boldmath$\psi$\unboldmath}}
\def\omegabf{\hbox{\boldmath$\omega$\unboldmath}}
\def\inftybf{\hbox{\boldmath$\infty$\unboldmath}}
\def\hSigmabf{\hbox{$\widehat{\bf \Sigma}$}}
\def\Sigmabf{\hbox{$\bf \Sigma$}}
\def\Upsilonbf{\hbox{$\bf \Upsilon$}}
%\def\Phibf{\hbox{$\bf \Phi$}}
%\def\Psibf{\hbox{$\bf \Psi$}}
\def\Omegabf{\hbox{$\bf \Omega$}}
\def\Deltabf{\hbox{$\bf \Delta$}}
\def\Gammabf{\hbox{$\bf \Gamma$}}
\def\Thetabf{\hbox{$\bf \Theta$}}
\def\Lambdabf{\mbox{$ \bf \Lambda $}}
\def\Xibf{\hbox{\bf$\Xi$}}
\def\Pibf{{\bf \Pi}}
%\def\thetabf{\hbox{\boldmath$\theta$\unboldmath}}
\def\thetabf{{\mbox{\boldmath$\theta$\unboldmath}}}
%\def\thetabf{\hbox{$\bf{\theta}$}}
\def\Upsilonbf{\hbox{\boldmath$\Upsilon$\unboldmath}}
\newcommand{\Phibf}{\mbox{${\bf \Phi}$}}
\newcommand{\Psibf}{\mbox{${\bf \Psi}$}}
\def\olambda{\mathfrak{o}(\lambda)}
\def\complex{\mathfrak{C}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Calligraphic
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
%\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%mathbb
\def\Abb{{\mathbb A}}
\def\BBb{{\mathbb B}}% different
\def\Cbb{{\mathbb C}}
\def\Dbb{{\mathbb D}}
\def\Ebb{{\mathbb E}}
\def\Fbb{{\mathbb F}}
\def\Gbb{{\mathbb G}}
\def\Hbb{{\mathbb H}}
\def\Ibb{{\mathbb I}}
\def\Jbb{{\mathbb J}}
\def\Kbb{{\mathbb K}}
\def\Lbb{{\mathbb L}}
\def\Mbb{{\mathbb M}}
\def\Nbb{{\mathbb N}}
\def\Obb{{\mathbb O}}
\def\Pbb{{\mathbb P}}
\def\Qbb{{\mathbb Q}}
\def\Rbb{{\mathbb R}}
\def\Sbb{{\mathbb S}}
\def\Tbb{{\mathbb T}}
\def\Ubb{{\mathbb U}}
\def\Vbb{{\mathbb V}}
\def\Wbb{{\mathbb W}}
\def\Xbb{{\mathbb X}}
\def\Ybb{{\mathbb Y}}
\def\Zbb{{\mathbb Z}}

\def\hbfP{{\widehat{\bfP}}}

\def\tilf{{\widetilde{f}}}

\def\tilo{{\widetilde{o}}}
\def\tilomega{{\widetilde{\omega}}}

\def\tilJbf{{\widetilde{\bfJ}}}

%\def\tilJ{{\widetilde{J}}}
\def\tilO{{\widetilde{O}}}
%\def\tilP{{\widetilde{P}}}
\def\tilR{{\widetilde{R}}}

\def\tilAbf{{\widetilde{\bfA}}}
\def\tilJbf{{\widetilde{\bfJ}}}
\def\tilRbf{{\widetilde{\bfR}}}


\def\tilEbb{{\widetilde{\Ebb}}}
\def\tilPbb{{\widetilde{\Pbb}}}


\def\tiltilEbb{{\widetilde{\widetilde{\Ebb}}}}
\def\tiltilP{{\widetilde{\widetilde{P}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%command abbreviations
\newcommand{\bprfof}{\begin{proof_of}}
\newcommand{\eprfof}{\end{proof_of}}
\newcommand{\bprf}{\begin{myproof}}
\newcommand{\eprf}{\end{myproof}}
\newcommand{\bp}{\begin{psfrags}}
\newcommand{\ep}{\end{psfrags}}
\newcommand{\bl}{\begin{lemma}}
\newcommand{\el}{\end{lemma}}
\newcommand{\bt}{\begin{theorem}}
\newcommand{\et}{\end{theorem}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}\noindent}
\def\beqn{\begin{eqnarray}}
\def\eeqn{\end{eqnarray} \noindent}
\def\beqnn{  \begin{eqnarray*}}
\def\eeqnn{\end{eqnarray*}  \noindent}
\def\bcase{  \begin{numcases}}
\def\ecase{\end{numcases}   \noindent}
\def\bsbcase{  \begin{subnumcases}}
\def\esbcase{\end{subnumcases}   \noindent}

\def\endproof{\hfill$\blacksquare$}
\def\defeq{{:=}}%{{\stackrel{\Delta}{=}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%theorems

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{A}
\newtheorem{properties}{Properties}
\newtheorem{conjecture}{Conjecture}
\newtheorem{criterion}{Criterion}
\newtheorem{proposition}{Proposition}
\newtheorem{notation}{Notation}
\newtheorem{derivation}{Derivation}
\newtheorem{claim}{Claim}
\newtheorem{observation}{Observation}
\newtheorem{fact}{Fact}

%\theoremstyle{definition}
\newtheorem{definition}{Definition}
%\theorembodyfont{\upshape} %body not italicized

%\theoremstyle{remark} %Comment it if you want to make the style of remarks the same as theorems
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
%\theoremheaderfont{\normalfont\bfseries}
%\theorembodyfont{\normalfont}
%\newtheorem{example}{Example}
%\newtheorem{proof}{Proof}

\newenvironment{myproof}{\noindent{\bf Proof:} \hspace*{1em}}{
    \hspace*{\fill} $\Box$ }
\newenvironment{proof_of}[1]{\noindent {\bf Proof of #1: }}{\hspace*{\fill} $\Box$ }
\newenvironment{proof_claim}{\begin{quotation} \noindent}{
    \hspace*{\fill} $\diamond$ \end{quotation}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\matplottc}[1]{               % single matlab plot twocolumn
        \unitlength .45truein
        \begin{center}
%         \begin{picture}(5,4.6)(1.05,.45)
        \special{psfile=#1.ps hscale=50 vscale=50}
        \end{picture}
        \end{center}
}
\newcommand{\matplotfp}[1]{               % single matlab plot fullpage
        \unitlength .45truein
        \begin{center}
        \begin{picture}(14,16)(.8,-1)
        \special{psfile=#1.ps hscale=100 vscale=100}
        \end{picture}
        \end{center}
}
\newcommand{\matplothp}[1]{               % single matlab plot halfpage
        \unitlength .45truein
        \begin{center}  \begin{picture}(14,7.5)(-1,.55)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplothptop}[1]{               % single matlab plot halfpage
        \unitlength .45truein                % when figure is top of page
        \begin{center}  \begin{picture}(14,6.3)(-1,1.15)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplotcc}[4]{             % two axis('square') plots side by side
        \vspace{2.8in}
        \special{psfile=#1.ps voffset=-10 hoffset=-22 vscale=52 hscale=52}
        \special{psfile=/user/xu/isl/matlab/psfiles/#2.ps voffset=-10 hoffset=213 vscale=52 hscale=52}
        \hspace*{\fill}\hspace*{0.35in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.35in}#4\hspace*{\fill} }
\newcommand{\matplottwo}[4]{             % two axis('normal') plots side by side
        \vspace{2.62in}
        \special{psfile=#1.ps voffset=-10 hoffset=-27 vscale=52 hscale=52}
        \special{psfile=#2.ps voffset=-10 hoffset=218 vscale=52 hscale=52}
        \vspace*{0.18in}
        \hspace*{\fill}\hspace*{-.05in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.65in}#4\hspace*{\fill} } %%
%% This is for making fancy paragraphs
%%
\def\psfancypar#1#2{\begingroup\def\par{\endgraf\endgroup\lineskiplimit=0pt}
               \setbox2=\hbox{\large\sc #2}
%              \showthe\lht2\showthe\baselineskip
               \newdimen\tmpht \tmpht \ht2 \advance\tmpht by \baselineskip
%              \showthe\tmpht
% Changed 10/2/89 rhr - t-bol -> Times-Bold for dvi2ps to dvips conversion
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
%              \showthe\ht1
               \count7=\tmpht \count8=\ht1
%  note that all this BS is necessary since TeX only does integer
%  divides and rounds all results
               \divide\count8 by 1000 \divide\count7 by \count8
%               \showthe\count7
               \tmpht=.001\tmpht\multiply\tmpht by \count7
%               \showthe\tmpht
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
               \noindent
                \hangindent1.05\wd1
               \hangafter=-2 {\hskip-\hangindent
               \lower1\ht1\hbox{\raise1.0\ht2\copy1}%
                \kern-0\wd1}\copy2\lineskiplimit=-1000pt}


\newenvironment{ap}{
\renewcommand{\thesection}{\mbox{Appendix }\Alph{section}}
\renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection
}}
\renewcommand{\theequation}{\mbox{\Alph{section}.}\arabic{equation}}
}{
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\theequation}{\arabic{equation}}
}



\def\Kout{\setbox1=\hbox{\Huge\bf K}\hbox to
1.05\wd1{\hspace{.05\wd1}\special{
"/Times-BoldItalic findfont 25 scalefont setfont
/prKzip
{0 0 moveto (K) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prKzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prKzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (K) true charpath  stroke
 grestore
} def
dozip}}}
\def\Sout{\setbox1=\hbox{\Huge\bf S}\hbox to 1.05\wd1{\hspace{.05\wd1}\special{"
/Times-BoldItalic findfont 25 scalefont setfont
/prSzip
{0 0 moveto (S) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prSzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prSzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (S) true charpath  stroke
 grestore
} def
dozip}}}
\newcommand{\hKbf}{\mbox{${\widehat{\bfK}}$}}
\newcommand{\hthetabf}{\mbox{${\widehat{\thetabf}}$}}
\newcommand{\hmubf}{\mbox{${\widehat{\mubf}}$}}
%\newcommand{\thbar}{\mbox{${\bar{\thetabf}}_N$}}
%\newcommand{\etahat}{\mbox{${\hat{\etabf}}$}}
%\newcommand{\etabf}{\mbox{${\bf\eta}$}}
%\newcommand{\e}{\mbox{${\bf e}_k$}}
%\newcommand{\ehat}{\mbox{$\hat{\bf e}_k$}}
%\newcommand{\EWE}{\mbox{${\bf E}_s^{}{\bf WE}_s^*$}}
%\newcommand{\DPD}{\mbox{$\Dbf^*\Pbf_{\bf A}^{\perp} \Dbf$}}
%\newcommand{\EWEhat}{\mbox{$\hat{\bf E}_s^{}{\bf W}\hat{\bf E}_s^*$}}
%\newcommand{\E}{\mbox{{\rm E}}}
%\newcommand{\Efs}{\mbox{${\bf E}_s^{}$}}
%\newcommand{\En}{\mbox{${\bf E}_n^{}$}}
%\newcommand{\Eshat}{\mbox{$\hat{\bf E}_s^{}$}}
%\newcommand{\Lshat}{\mbox{$\hat {\bf \Lambda}_s^{}$}}
%\newcommand{\Ls}{\mbox{$ {\bf \Lambda}_s^{}$}}
%\newcommand{\Ln}{\mbox{$ {\bf \Lambda}_n^{}$}}
%\newcommand{\Ltilde}{\mbox{$\widetilde {\bf \Lambda}$}}
%\newcommand{\Enhat}{\mbox{$\hat{\bf E}_n^{}$}}
%\newcommand{\Lnhat}{\mbox{$\hat {\bf \Lambda}_n^{}$}}
%\newcommand{\Ai}{\mbox{$ ({\bf A}^*{\bf A})^{-1} $}}
%\newcommand{\abf}{\mbox{${\bf a}$}}


%Define affiliation at footnote
% Make \small be smaller (8 pt)
%\def\small{\@setsize\small{9pt}\viiipt\@viiipt\let\@listi\@listI}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros to restate theorems in appendices
%
% Use as follows:
%\torestate{Theorem}{thm:restate}{If $x \in \N$ then $x+1 \in \N$.}
%
%\restate{thm:restate}

\newcommand{\torestate}[3]{%
\expandafter \def \csname BBRESTATE #2 \endcsname{#3}
\theoremstyle{plain}
\newtheorem{BBRESTATETHMNUM#2}[theorem]{#1}
\begin{BBRESTATETHMNUM#2}\label{#2}\csname BBRESTATE #2 \endcsname   \end{BBRESTATETHMNUM#2}
\newtheorem*{BBRESTATETHMNONNUM#2}{{#1}~\ref{#2}}
}


\newcommand{\restate}[1]{\begin{BBRESTATETHMNONNUM#1}[Restated] \csname BBRESTATE #1 \endcsname
\end{BBRESTATETHMNONNUM#1}}


\definecolor{blue1}{HTML}{0066FF}
\definecolor{lpurple}{cmyk}{.05,0.18,0,0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> maintable.tex <==
\section{Table of Content}

\begin{table}[htbp]\vspace{-1cm}\caption{Table of Notation My Research}
\begin{center}% used the environment to augment the vertical space
% between the caption and the table
\begin{tabular}{r c p{10cm} }
\toprule

$\X$ &  & Finite state space \\
$\Y$ &  & Finite observation space\\ 
$\A$ &  & Finite action space \\  
$\R$ &  & Finite reward space\\  
$X$ &  & Cardinality of state space\\  
$Y$ &  & Cardinality of observation space\\  
$A$ &  & Cardinality of action space\\  
$R$ &  & Cardinality of reward space\\  
$r_{\max}$ &  & Largest reward\\  
$x$ &  & state indicator random variable\\  
$\vec{y}$ &  & observation indicator random variable\\  
$r$ &  & reward indicator random variable\\
$a~or~l$ &  & action indicator random variable\\    
$T$ &  & Transition tensor \\  
$O$ &  & Observation matrix\\  
$\Gamma$ &  & Reward tensor\\
$\Pi$ &  & Policy matrix\\
$M$ &  & POMDP model\\
$\M^{(k)}$ &  & Set of plausible POMDP at episode $k$\\
$f_T(x'|x,a)$ &  & transition density from state $x$ to state $x'$ given action $a$\\  
$f_O(\vec{y}|x)$ &  & observation density\\  
$f_R(r|x,a)$ &  & reward density given pair of state-action\\  
$f_T(x'|x)$ &  & corresponding Markov chain transition density\\  
$\calP$ &  & Set of all plausible stochastic memory-less policies\\  
$\pi$ &  & memory less policy, observation $\rightarrow$ action\\  
$\pi_{\min}$ &  & smallest element of policy matrix memory-less policy, observation $\rightarrow$ action\\  
$\eta(\pi,M)$ &  & expected average reward given model and policy\\    
$\omega_\pi$ &  & vector of stationary distribution over states given policy $\pi $ \\  
$\vec{v}_{i,t}^{(l)}$ &  & $i'th$ view at time t give $a_t=l$(middle action= $l$), $i\in\{1,2,3\}$\\  
$V_{\nu}^{(l)}$ &  & $\nu'th$ View matrix representation $\nu\in\{1,2,3\}$\\  
$K_{\nu,\nu'}^{(l)}$ &  & Covariance matrix between view $\nu$ and $\nu'$, where $\nu,nu'\in\{1,2,3\}$ given middle action $l$\\  
$M_2^{(l)}$ &  & Second order moment given middle action $l$\\  
$M_3^{(l)}$ &  & Third order moment given middle action $l$\\
$\sigma_{\nu,\nu'}^{(l)}$ &  & smallest non-zero singular value of covariance matrix of views $\nu$ and $\nu'$ given middle action $l$ \\  
$C_O, C_R, C_T$ &  & Suitable numerical constants\\  
$N$ &  & Number of total samples\\  
$N(l)$ &  & Number of triple with middle action $l$\\    
$D$ &  & The model diameter\\
$\B_O$ &  & Upper confidence bound over error of estimated $f_O$\\  
$\B_R$ &  & Upper confidence bound over error of estimated $f_R$\\  
$\B_T$ &  & Upper confidence bound over error of estimated $f_T$\\

\bottomrule
\end{tabular}
\end{center}
\label{tab:TableOfNotationForMyResearch}
\end{table}



==> maintable_short.tex <==
% !TEX root = master.tex

\section{Table of Notation}\label{s:notation}

%\vspace{-1cm}
\begin{table}[htbp]%\caption{Main notation used throughout the paper.}
\begin{center}% used the environment to augment the vertical space
% between the caption and the table
\begin{small}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{r c p{12.3cm} }
\toprule

\multicolumn{3}{c}{\textbf{POMDP Notation} (Sect.~\ref{s:preliminaries})}\\
\midrule
$\vec{e}$ &  & indicator vector \\
$M$ &  & POMDP model\\
$\X, X, x, (i,j)$ &  & state space, cardinality, element, indices \\
$\Y, Y, \vec{y}, n$ &  & observation space, cardinality, indicator element, index \\
$\A, A, a, (l, k)$ &  & action space, cardinality, element, indices \\
$\R, R, r, \vec{r}, m, r_{\max}$ &  & reward space, cardinality, element, indicator element, index, largest value \\
$f_T(x'|x,a), T$ &  & transition density from state $x$ to state $x'$ given action $a$ and transition tensor\\  
$f_O(\vec{y}|x), O$ &  & observation density of indicator $\vec{y}$ given state $x$ and observation matrix\\  
$f_R(\vec{r}|x,a), \Gamma$ &  & reward density of indicator $\vec{r}$ given pair of state-action and reward tensor\\  
$\pi, f_\pi(a|\vec{y}), \Pi$ &  & policy, policy density of action $a$ given observation indicator $\vec{y}$ and policy matrix\\  
$\pi_{\min}$, $\calP$ &  & smallest element of policy matrix and set of stochastic memoryless policies\\  
$f_{\pi,T}(x'|x)$ &  & Markov chain transition density for policy $\pi$ on a POMDP with transition density $f_T$\\  
$\omega_\pi$, $\omega_\pi^{(l)}$ &  & stationary distribution over states given policy $\pi$ and conditional on action $l$ \\  
$\eta(\pi,M)$ &  & expected average reward of policy $\pi$ in POMDP $M$\\    
$\eta^+$ &  & best expected average reward over policies in $\calP$\\    
& & \\
\multicolumn{3}{c}{\textbf{POMDP Estimation Notation} (Sect.~\ref{s:learning.pomdp})}\\
\midrule
$\nu\in\{1,2,3\}$ & & index of the views\\
$\vec{v}_{\nu,t}^{(l)}$, $V_{\nu}^{(l)}$ &  & $\nu$th view and view matrix at time $t$ given $a_t=l$\\
$K_{\nu,\nu'}^{(l)}$, $\sigma_{\nu,\nu'}^{(l)}$ &  & covariance matrix of views $\nu, \nu'$ and its smallest non-zero singular value given action $l$\\
%$\sigma_{\nu,\nu'}^{(l)}$ &  &  of $K_{\nu,\nu'}^{(l)}$\\
$M_2^{(l)}$, $M_3^{(l)}$ &  & second and third order moments of the views given middle action $l$\\  
$\wh{f}_O^{(l)}$, $\wh{f}_R^{(l)}$, $\wh{f}_T^{(l)}$ &  & estimates of observation, reward, and transition densities for action $l$\\  
$N$, $N(l)$ &  & total number of samples and number of samples from action $l$\\  
$C_O, C_R, C_T$ &  & numerical constants\\  
$\B_O$, $\B_R$, $\B_T$ &  & upper confidence bound over error of estimated $f_O$, $f_R$, $f_T$\\  
& & \\
\multicolumn{3}{c}{\textbf{\smucrl} (Sect.~\ref{s:learning})}\\
\midrule
$\text{Reg}_N$ & & cumulative regret \\
$D$ &  & POMDP diameter\\
$k$ & & index of the episode\\
$\wh{f}_T^{(k)}, \wh{f}_R^{(k)}, \wh{f}_O^{(k)}$, $\wh{M}^{(k)}$ & & estimated parameters of the POMDP at episode $k$ \\
$\M^{(k)}$ &  & set of plausible POMDPs at episode $k$\\
$v^{(k)}(l)$ &  & number of samples from action $l$ in episode $k$ \\
$N^{(k)}(l)$ &  & maximum number of samples from action $l$ over all episodes before $k$ \\
$\wt{\pi}^{(k)}$ &  & optimistic policy executed in episode $k$ \\
$\wb{N}$ & & min. number of samples to meet the condition in Thm.~\ref{thm:estimates} for any policy and any action \\
$\wb{\sigma}_{\nu,\nu'}$ & & worst smallest non-zero singular value of covariance $K_{\nu,\nu'}^{(l)}$ for any policy and action \\
$\wb{\omega}_{\min}$ & & smallest stationary probability over actions, states, and policies \\

\bottomrule
\end{tabular}
\end{small}
\end{center}
\label{tab:notation.small}
\end{table}


